Multi-modality fusion using canonical correlation analysis methods: Application in breast cancer survival prediction from histology and genomics

The availability of multi-modality datasets provides a unique opportunity to characterize the same object of interest using multiple viewpoints more comprehensively. In this work, we investigate the use of canonical correlation analysis (CCA) and penalized variants of CCA (pCCA) for the fusion of two modalities. We study a simple graphical model for the generation of two-modality data. We analytically show that, with known model parameters, posterior mean estimators that jointly use both modalities outperform arbitrary linear mixing of single modality posterior estimators in latent variable prediction. Penalized extensions of CCA (pCCA) that incorporate domain knowledge can discover correlations with high-dimensional, low-sample data, whereas traditional CCA is inapplicable. To facilitate the generation of multi-dimensional embeddings with pCCA, we propose two matrix deflation schemes that enforce desirable properties exhibited by CCA. We propose a two-stage prediction pipeline using pCCA embeddings generated with deflation for latent variable prediction by combining all the above. On simulated data, our proposed model drastically reduces the mean-squared error in latent variable prediction. When applied to publicly available histopathology data and RNA-sequencing data from The Cancer Genome Atlas (TCGA) breast cancer patients, our model can outperform principal components analysis (PCA) embeddings of the same dimension in survival prediction.

==> commands.tex <==
% \IEEEoverridecommandlockouts    
% \let\labelindent\relax
% % \usepackage{enumitem}
% \usepackage{amsthm}
\usepackage{mathtools}
% \usepackage{amsmath}
\usepackage{amsfonts,amssymb,url} % \usepackage{cite}
% \usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{setspace}
\usepackage{comment}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{adjustbox}
% % \usepackage{graphicx}
% % \usepackage{textcomp}
% \usepackage{setspace}
% % \usepackage{color}
% % \usepackage{epsfig}  % for figures
% %\usepackage{graphicx}  % another package that works for figures
% %\usepackage{subfigure}  % for subfigures
%  % for math spacing
\usepackage{amssymb}  % USE FOR MEDIA
% \usepackage{url}  % Hyphenation of URLs.
% \usepackage{lscape}  % Useful for wide tables or figures.
% % \usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{float,graphicx}
% % \usepackage{subcaption}
\usepackage[english]{babel}
\usepackage[ruled,vlined]{algorithm2e}
% \usepackage{bbm,tikz}
% \usepackage{prettyref,xspace}
% \usepackage{enumitem}
% \usepackage{cite}
% \usepackage{multirow}
% %\usepackage[style=numeric-comp,subentry,backend=biber]{biblatex}

% \newcommand{\figref}[1] {{Fig.\ref{#1}}}

% \usepackage{tkz-graph}
% \GraphInit[vstyle = Shade]
% \tikzset{
%   LabelStyle/.style = { rectangle, rounded corners, draw,
%                         minimum width = 2em, fill = yellow!50,
%                         text = red, font = \bfseries },
%   VertexStyle/.append style = { inner sep=5pt,
%                                 font = \normalsize\bfseries},
%   EdgeStyle/.append style = {->, bend left} }
% \usetikzlibrary {positioning,shapes,arrows}


% \newrefformat{eq}{(\ref{#1})}
% \newrefformat{thm}{Theorem~\ref{#1}}
% \newrefformat{th}{Theorem~\ref{#1}}
% \newrefformat{chap}{Chapter~\ref{#1}}
% \newrefformat{sec}{Section~\ref{#1}}
% \newrefformat{algo}{Algorithm~\ref{#1}}
% \newrefformat{fig}{Figure.~\ref{#1}}
% \newrefformat{tab}{Table~\ref{#1}}
% \newrefformat{rmk}{Remark~\ref{#1}}
% \newrefformat{clm}{Claim~\ref{#1}}
% \newrefformat{def}{Definition~\ref{#1}}
% \newrefformat{cor}{Corollary~\ref{#1}}
% \newrefformat{lmm}{Lemma~\ref{#1}}
% \newrefformat{prop}{Proposition~\ref{#1}}
% \newrefformat{pr}{Proposition~\ref{#1}}
% \newrefformat{app}{App $\hat{z}_C$ endix~\ref{#1}}
% \newrefformat{ques}{Question~\ref{#1}}

% \newcommand{\distR}{\mathrm{dist}_R}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
% \newcommand{\sgn}{\text{sgn}}

% %% parenthesis
% \newcommand{\pth}[1]{\left( #1 \right)}
% \newcommand{\qth}[1]{\left[ #1 \right]}
% \newcommand{\sth}[1]{\left\{ #1 \right\}}
% \newcommand{\floor}[1]{{\left\lfloor {#1} \right \rfloor}}
% \newcommand{\ceil}[1]{{\left\lceil {#1} \right \rceil}}
% \newcommand{\eg}{e.g.\xspace}
% \newcommand{\ie}{i.e.\xspace}
% \newcommand{\iid}{i.i.d.\xspace}


\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{proof}{Proof}
\newtheorem{corollary}{Corollary}
\newtheorem{coro}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{prop}{Proposition}
% \newtheorem{proofpart}{Step}


% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
% \newtheorem{remark}{Remark}
% \newtheorem{question}{Question}
% %\newcommand{}{\displaystyle}
% \newcommand{\lk} { \lim_{k \rightarrow \infty}}

% \newcommand{\Z}{\mathbb{Z}}
% \newcommand{\A}{\\[0.2em]}
% \newcommand{\AC}{\mathcal{A}}
% \newcommand{\BC}{\mathcal{B}}
% \newcommand{\ZC}{\mathcal{Z}}
% \newcommand{\TV}{d_\mathrm{TV}}

% \newcommand{\red}{\color{red}}
% \newcommand{\blue}{\color{blue}}
% \newcommand{\nb}[1]{{\sf\blue[#1]}}
% \newcommand{\nbr}[1]{{\sf\red[#1]}}
% \newcommand{\Mod}[1]{\ (\text{mod}\ #1)}

% \newcommand{\torus}{\mathbb{T}}
% \newcommand{\diverge}{\to\infty}
% \newcommand{\reals}{\mathbb{R}}
% \newcommand{\naturals}{\mathbb{N}}
% \newcommand{\integers}{\mathbb{Z}}
% \newcommand{\Expect}{\mathbb{E}}
% \newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
% \newcommand{\Prob}{\mathbb{P}}
% \newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
% \newcommand{\pprob}[1]{\mathbb{P}[#1]}
% \newcommand{\calU}{\mathcal{U}}
% \newcommand{\calL}{\mathcal{L}}


% %My own custom made

% \newcommand{\hyy}{\hat{Y}}
% \newcommand{\hy}{\hat{y}}
% \newcommand{\soft}{\mathrm{softmax}}
% \newcommand{\derv}[2]{\frac{\partial{#1}}{\partial {#2}}}
% \newcommand{\tilh}{\tilde{h}}
% \newcommand{\diag}[1]{\mathrm{diag}(#1)}
% \newcommand{\add}{\sum_{j=1}^m}
% %\newcommand{\add}[3]{\sum_{#1=#2}^{#3}}
% %\newcommand{\mathbb{•}mat}[2]{\reals^{#1 \times #2}}
% \newcommand{\unif}{\mathrm{Unif}}
% \newcommand{\poi}{\mathrm{Poi}}
 
% % Common commands and definitions

% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{latexsym}
% \usepackage{verbatim}
% %\usepackage{subfigure}
% %\usepackage[final]{graphicx}
% \usepackage{psfrag}
% \usepackage{epsfig}
% % \usepackage{xcolor}
% % \usepackage{subfig}
% %\usepackage[•]{•}
% \usepackage[ruled,vlined]{algorithm2e}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output} 
\SetKwInput{KwParameters}{Parameters} 
% % %===========================================================================
% % % SPECIFIC STUFF USED FOR GENERATION OF DRAFT:
% % %
% % %\usepackage{drafthead}       % draft version printed at top of page.
% % %\usepackage{showkeys}        % show labels and references.
% %
% % % Use one-and-one-helf spacing
% % \linespread{1.25}
% %
% % % Set paper size to full page (based on fullpage.sty).
% % \topmargin 0pt
% % \advance \topmargin by -\headheight
% % \advance \topmargin by -\headsep
% % \textheight 8.9in
% % \oddsidemargin 0pt
% % \evensidemargin \oddsidemargin
% % \marginparwidth 0.7in
% % \textwidth 6.5in

% % Incorporate the above by using \usepackage{bbc_sizes}
% % in main.tex. Changed by YB to allow using bbc.sty for slides.
% %===========================================================================
% %  COMMENTS AND REVISIONS:
% %
% %       {comment}       for comments to the other authors
% %       {later}         for things that need to be completed later
% %       \annote{text}   put annotation for other authors in the margin
% %       \scomment{text} for short comments ``inline''
% %       \source{ref}    reference for the material (not printed)
% %
% % Allow comments and marginal notes to be integrated
% % in the text or in the margin in distinct font.
% %
% %\newenvironment{comment}{\sffamily\itshape\small}{}
% %\newenvironment{later}{\begin{comment}\mbox{}\\[1ex]}{\\[1ex]\null\end{comment}}
% %%\marginparwidth=1.7cm
% %\newcommand{\scomment}[1]{\begin{comment}#1\end{comment}}
% %\newcommand{\annote}[1]{\begin{comment}\marginpar{\raggedright\sffamily\itshape\scriptsize #1}\end{comment}}
% %\newcommand{\source}[1]{}



% %===========================================================================
% % THEOREMS AND RELATED ENVIRONMENTS
% %
% %       {theorem}       for statement of theorems
% %       {lemma}         for statement of lemmas
% %       {corollary}     for statement of corollaries
% %       {conjecture}    for statement of conjectures
% %       {remark}        for remarks (not numbered)
% %       {note}          similar to remarks
% %       {definition}    for mathematical definition
% %       {example}       for numbered ``mathematical'' examples
% %       {illustration}  for ``dsp'' examples (not numbered)
% %       {proof}         for proofs of theorems. Ends with a QED symbol.
% %       {property}      for properties (simple, not in theorems)
% %
% % Based on amsthm package
% %
% % The environment {proof} is directly provided by the amsthm package.
% %
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% %\newtheorem{corollary}{Corollary}
% \newtheorem{property}{Property}
% %\theoremstyle{definition}
% %\newtheorem{definition}{Definition}
% \newtheorem{conjecture}{Conjecture}
% %\theoremstyle{remark}
% %\newtheorem{remark}{Remark} % not numbered
% %\newtheorem{note}{Note} % not numbered

% %\newtheoremstyle{illustration}{24pt}{24pt}{\sf \small}{}{\bf \normalsize \sc}{:}{10pt}{}
% %\theoremstyle{illustration}
% \newtheorem{illustration}{Illustration}
% %\newtheorem{example}{Example}

% %===========================================================================
% % END OF CHAPTER PROBLEMS:
% %
% %       {problems}      for problems at the end of each chapter
% %
% %
% % A chapter should be concluded with
% %               ....
% %               \begin{problems}
% %               \item Statement of first problem
% %               \item ...
% %               \end{problems}
% %
% % TO DO LATER: define counter for chapter-based numbering in the
% % enumerate environment (new list environment).
% %
% \newenvironment{problems}{\section*{Problems}\begin{enumerate}}{\end{enumerate}}
% \newenvironment{problemsec}{\section{Problems}\begin{enumerate}}{\end{enumerate}}
% %===========================================================================
% % REFERENCE MANAGEMENT:
% %
% %       \refeq{label}   generate reference to (\label{eq:label})
% %       \refEq{label}   generate reference to Equation (\label{eq:label})
% %       \reffig{label}  generate reference to figure \label{fig:label}
% %       \refFig{label}  generate reference to Figure \label{fig:label}
% %       \reftab{label}  generate reference to table \label{tab:label}
% %       \refTab{label}  generate reference to Table \label{tab:label}
% %       \refsec{label}  generate reference to section \label{sec:label}
% %       \refSec{label}  generate reference to Section \label{sec:label}
% %       \refchap{label} generate reference to chapter \label{chap:label}
% %       \refChap{label} generate reference to Chapter \label{chap:label}
% %       \refpart{label} generate reference to part \label{part:label}
% %       \refPart{label} generate reference to Part \label{part:label}
% %       \refthm{label}  generate reference to theorem \label{thm:label}
% %       \refThm{label}  generate reference to Theorem \label{thm:label}
% %       \refcor{label}  generate reference to corrolary \label{cor:label}
% %       \refCor{label}  generate reference to Corrolary \label{cor:label}
% %       \refprp{label}  generate reference to property \label{prp:label}
% %       \refPrp{label}  generate reference to Property \label{prp:label}
% %
% % Associated convention: labels should be ``typed casted''. Example:
% % \label{eq:Cauchy} for an equation, \label{fig:SNR} for a figure,
% % or \label{tab:performance} for a table.
% % Reference are ``type casted'' by the macro. Example:
% % Equation \refeq{Cauchy} or \reffig{SNR}.
% %
% % Labels are of the form eq:XXX_tag, where the first part identifies the
% % type of object, the second part identifies the chapter (3 capital letters,
% % and the last part identifies the object inside the chapter).

% \newcommand{\refeq}[1]{\eqref{eq:#1}}  % call \eqref from amstex
% \newcommand{\refEq}[1]{Equation \eqref{eq:#1}}
% \newcommand{\reffig}[1]{figure~\ref{fig:#1}}
% \newcommand{\refFig}[1]{Figure~\ref{fig:#1}}
% \newcommand{\reftab}[1]{table~\ref{tab:#1}}
% \newcommand{\refTab}[1]{Table~\ref{tab:#1}}
% \newcommand{\refsec}[1]{section~\ref{sec:#1}}
% \newcommand{\refSec}[1]{Section~\ref{sec:#1}}
% \newcommand{\refchap}[1]{chapter~\ref{chap:#1}}
% \newcommand{\refChap}[1]{Chapter~\ref{chap:#1}}
% \newcommand{\refpart}[1]{part~\ref{part:#1}}
% \newcommand{\refPart}[1]{Part~\ref{part:#1}}
% \newcommand{\refthm}[1]{theorem~\ref{thm:#1}}
% \newcommand{\refThm}[1]{Theorem~\ref{thm:#1}}
% \newcommand{\refcor}[1]{corrolary~\ref{cor:#1}}
% \newcommand{\refCor}[1]{Corrolary~\ref{cor:#1}}
% \newcommand{\refprp}[1]{property~\ref{prp:#1}}
% \newcommand{\refPrp}[1]{Property~\ref{prp:#1}}
% \newcommand{\refdef}[1]{definition~\ref{def:#1}}
% \newcommand{\refDef}[1]{Definition~\ref{Def:#1}}
% \newcommand{\refProb}[1]{Problem~\ref{Prob:#1}}
% % \newcommand{\refEx}[1]{Example~\ref{ex:#1}}
% %===========================================================================
% % MATHEMATICAL SYMBOLS AND NOTATIONS

% % ``Formatting'' command
% %
% %       \Ma{A}          matrix
% %       \Ve{x}          vector
% %       \Op{A}          operator
% %       \St{A}          set
% %       \Sc{A}          space or subspace
% %       \Range(A)       range of A
% %       \Null(A)        nullspace of A
% %       A^\Trans        A transpose
% %       A^\Herm         A Hermitian transpose
% %       A^\Adj          A adjoint
% %       A^\LS           A least-square
% %       A^\MN           A mininum-norm
% %       A^\MNLS         A mininum-norm least-squares
% %       A^\LI           left inverse of A
% %       A^\RI           right inverse of A
% %       A^\Pinv         pseudo-inverse of A
% %
\newcommand{\Ma}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Ve}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Op}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Set}[1]{\ensuremath{{#1}}}
\newcommand{\Spc}[1]{\ensuremath{#1}}
\newcommand{\Range}{R}
\newcommand{\Null}{N}
\newcommand{\Trans}{T}
\newcommand{\Herm}{H}
\newcommand{\Adj}{*}
\newcommand{\LS}{\mathrm{LS}}
\newcommand{\MN}{\mathrm{MN}}
\newcommand{\MNLS}{\mathrm{MNLS}}
\newcommand{\LI}{L}
\newcommand{\RI}{R}
\newcommand{\Pinv}{\dagger}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\mLambda}{\boldsymbol{\Lambda}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
% % Useful symbols and operators not defined in AMS-LaTeX
% %
% %       \Natural        set of positive integersx
% %       \Integer        set of integers
% %       \Real           real line
% %       \Complex        complex space
% %       \Poly           space of polynomials
% %       \indep          statistical independence operator
% %       \defeq          definition operator
% %       \aeeq           a.e. equality operator
% %       \var            variance operator
% %       \cov            covariance operator
% %       \rank           rank operator
% %       \Trace          trace operator tr
% %       \Span           span operator
% %       \toeplitz       Toeplitz matrix operator
% %       \block          block operator
% %       \dif            integration: \int x^2 \dif{x}
% %       \comp           set complement \comp{\Set{S}}
% %       \Conj           Conjugate \Conj{x}
% %
\newcommand{\Natural}{\ensuremath{\mathbb{N}}}
\newcommand{\Integer}{\ensuremath{\mathbb{Z}}}
\newcommand{\Real}{\ensuremath{\mathbb{R}}}
\newcommand{\Complex}{\ensuremath{\mathbb{C}}}
\newcommand{\C}{\Complex}
\newcommand{\R}{\Real}
\newcommand{\inv}[1]{{#1}^{-1}}
% \newcommand{\Rational}{\ensuremath{\mathbb{Q}}}
% \newcommand{\Poly}{\mathbb{P}}
% \newcommand{\inprod}[1]{\langle{#1}\rangle}
% \newcommand{\indep}{\mathop{\perp\hspace*{-.65em}\perp}\limits}
% \newcommand{\defeq}{\mathbin{\stackrel{\bigtriangleup}{=}}}
% \newcommand{\aeeq}{\mathbin{\stackrel{\mathrm{a.e.}}{=}}}
% \newcommand{\comp}[1]{#1^c}
% \newcommand{\Conj}[1]{\bar{#1}}
% \DeclareMathOperator{\var}{Var} \DeclareMathOperator{\cov}{Cov}
% %\DeclareMathOperator{\diag}{diag}
% \DeclareMathOperator{\rank}{rank} 
\DeclareMathOperator{\Trace}{tr}
% \DeclareMathOperator{\Span}{span}
% \DeclareMathOperator{\Sign}{sign}
% \DeclareMathOperator{\toeplitz}{Toeplitz}
% \DeclareMathOperator{\block}{block}
% \newcommand{\dif}{\,d}

% % Inner product, abs, norm, etc, with automatique size adaptation.
% % May need the addition of \right. and \left. in its arguments in
% % some situations
% % In case of hand coding, use \bigl, \bigr, \Bigl, \Bigr, \Bigl, \Bigr,
% % \biggl, \biggr, \Biggl, \Biggr
% % Usage:  \norm{x}\norm{y}\leq\ip{x}{y}

% \newcommand{\lacute}{\mathopen{<}} % Delimiters for inner-products <x,y>
% \newcommand{\racute}{\mathclose{>}}
%  \newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
% % \newcommand{\twonorm}[1]{\left\Vert#1\right\Vert_{2}}
% \newcommand{\twonorm}[1]{\left\Vert#1\right\Vert}
% %===========================================================================
% % SHORTCUTS:
% % Most of the shortcuts can be used both in text mode and
% % in math mode (\ensuremath), be careful with spacing though.
% % a good thing is probably to add {} after the command in text mode.

% % Common matrices and vectors
\newcommand{\mA}{\Ma{A}}
\newcommand{\mB}{\Ma{B}}
\newcommand{\mF}{\Ma{F}}
\newcommand{\mI}{\Ma{I}}
\newcommand{\mJ}{\Ma{J}}
\newcommand{\mK}{\Ma{K}}
\newcommand{\mL}{\Ma{L}}
\newcommand{\mM}{\Ma{M}}
\newcommand{\mP}{\Ma{P}}
\newcommand{\mQ}{\Ma{Q}}
\newcommand{\mT}{\Ma{T}}
\newcommand{\va}{\Ve{a}}
\newcommand{\vb}{\Ve{b}}
\newcommand{\vc}{\Ve{c}}

\newcommand{\vl}{\Ve{l}}
\newcommand{\vp}{\Ve{p}}
\newcommand{\vq}{\Ve{q}}
\newcommand{\vr}{\Ve{r}}
\newcommand{\vs}{\Ve{s}}
\newcommand{\vu}{\Ve{u}}
\newcommand{\vv}{\Ve{v}}
\newcommand{\vx}{\Ve{x}}
\newcommand{\vy}{\Ve{y}}
\newcommand{\vz}{\Ve{z}}
\newcommand{\vzero}{\Ve{0}}
% \newcommand{\valpha}{\Ve{0}}

% % Dot product (matrix)
% \newcommand{\dotp}[2]{\ensuremath{#1^\Herm #2}}

% % Symbols
% \newcommand{\FA}{~\forall~}

% % Calligraphic capitals
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
%\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
%\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Y}}}

% % Bold greek symbols
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bvarpi}{\boldsymbol{\varpi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\bvarsigma}{\boldsymbol{\varsigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\mathb}[1]{\boldsymbol{#1}}
\newcommand{\bGamma}{{\mathb{\Gamma}}}
\newcommand{\bDelta}{{\mathb{\Delta}}}
\newcommand{\bTheta}{{\mathb{\Theta}}}
\newcommand{\bLambda}{{\mathb{\Lambda}}}
\newcommand{\bXi}{{\mathb{\Xi}}}
\newcommand{\bPi}{{\mathb{\Pi}}}
\newcommand{\bSigma}{{\mathb{\Sigma}}}
\newcommand{\bUpsilon}{{\mathb{\Upsilon}}}
\newcommand{\bPhi}{{\mathb{\Phi}}}
\newcommand{\bPsi}{{\mathb{\Psi}}}
\newcommand{\bOmega}{{\mathb{\Omega}}}


% % New commands to be sorted into this hierarchy: skb 1/30/2000
% \newcommand{\conv}{\ast}
% \newcommand{\circconv}[1]{\circledast_{#1}}
% \newcommand{\Reverse}[1]{{#1}^{\text{R}}}
% \newcommand{\Thresh}{\text{Thresh}}
% \renewcommand{\Range}[1]{\mathrm{R}(#1)}
% \renewcommand{\Null}[1]{\mathrm{N}(#1)}
% \newcommand{\Spanp}[1]{\mathrm{span}(#1)}
% \newcommand{\Spanbig}[1]{\mathrm{span}\left\{ #1 \right\}}
% \newcommand{\Spanb}[1]{\mathrm{span}\{ #1 \}}
% \newcommand{\refill}[1]{illustration~\ref{ill:#1}}
% \newcommand{\refIll}[1]{Illustration~\ref{ill:#1}}
% \newcommand{\refex}[1]{example~\ref{ex:#1}}
% \newcommand{\refEx}[1]{Example~\ref{ex:#1}}
% \newcommand{\modN}[1]{<#1>_{N}}
% \newcommand{\vn}{\Ve{n}}
% \renewcommand{\to}{\implies}
% \renewcommand{\refcor}[1]{corollary~\ref{cor:#1}}
% \renewcommand{\refCor}[1]{Corollary~\ref{cor:#1}}
% \renewcommand{\refdef}[1]{definition~\ref{def:#1}}
% \renewcommand{\refDef}[1]{Definition~\ref{def:#1}}
% \newcommand{\bb}{\begin{bmatrix}}
% \newcommand{\eb}{\end{bmatrix}}
% \newcommand{\cj}{\jmath}
% \renewcommand{\Spc}[1]{\ensuremath{{\cal #1}}}
% \newcommand{\intersect}{\cap}
\newcommand{\mC}{\Ma{C}}
\newcommand{\vt}{\Ve{t}}
% \newcommand{\refssec}[1]{Subsection~\ref{ssec:#1}}
% \newcommand{\VEC}[1]{{\text{vec}}(#1)}
\newcommand{\mD}{\Ma{D}}
\newcommand{\mW}{\Ma{W}}
% \newcommand{\mtU}{\tilde{\Ma{U}}}
% \newcommand{\mtSigma}{\tilde{\Ma{\Sigma}}}
% \newcommand{\mtV}{\tilde{\Ma{V}}}
% \newcommand{\mtX}{\tilde{\Ma{X}}}
% \newcommand{\ve}{\Ve{e}}
% \newcommand{\vw}{\Ve{w}}
% \newcommand{\union}{\cup}
% \newcommand{\snorm}[1]{\| #1 \|_2}
% \newcommand{\fnorm}[1]{\| #1 \|_{\mathrm F}}
\renewcommand{\Trace}[1]{\mathrm{tr}\left[#1\right]}

\newcommand{\mU}{\Ma{U}}
\newcommand{\mV}{\Ma{V}}
\newcommand{\mE}{\Ma{E}}
\newcommand{\mZ}{\Ma{Z}}
\newcommand{\mX}{\Ma{X}}
\newcommand{\mY}{\Ma{Y}}
\newcommand{\mG}{\Ma{G}}
\newcommand{\mS}{\Ma{S}}
\newcommand{\mH}{\Ma{H}}
% \newcommand{\mSigma}{\Ma{\Sigma}}
% \newcommand{\mZero}{\Ma{0}}
% \newcommand{\vv}{\Ve{v}}
% \newcommand{\vf}{\Ve{f}}
% \newcommand{\vg}{\Ve{g}}
% \newcommand{\vh}{\Ve{h}}
% \newcommand{\vomega}{\Ve{\omega}}
% \newcommand{\vtheta}{\Ve{\theta}}
% \newcommand{\Fnorm}[1]{\norm{#1}_\mathrm{F}}
% \newcommand{\Snorm}[1]{\norm{#1}_\mathrm{S}}
% \newcommand{\cond}[1]{\kappa(#1)}
% \newcommand{\mbyn}{\ensuremath{m \times n}}
% \newcommand{\reflem}[1]{lemma~\ref{lem:#1}}
% \newcommand{\refLem}[1]{Lemma~\ref{lem:#1}}
% % Kludge
% \newcommand{\Dim}[1]{\mathrm{dim}(#1)}
% \newcommand{\Rank}[1]{\mathrm{rank}(#1)}
% \newcommand{\Diag}[1]{\mathrm{diag}(#1)}
% \newcommand{\TLS}{\mathrm{TLS}}
% %\newcommand{\Expect}[1]{\mathrm{E}\left[#1\right]}
% \newcommand{\Nullp}[1]{\mathrm{N}^{\perp}(#1)}
% \newcommand{\Rangep}[1]{\mathrm{R}^{\perp}(#1)}
% \newcommand{\Cn}{\Complex^{n}}
% \newcommand{\Cm}{\Complex^{m}}
% \newcommand{\Cmn}{\Complex^{m \times n}}
% \newcommand{\Cnn}{\Complex^{n \times n}}

% \newcommand{\vlambda}{\boldsymbol{\lambda}}
% \newcommand{\mK}{\Ma{K}}
\newcommand{\mR}{\Ma{R}}
% \newcommand{\mtY}{\tilde{\Ma{Y}}}
% \newcommand{\Det}[1]{\mathrm{det}\left[#1\right]}
% \newcommand{\Fld}{\mathbb{F}}
% \newcommand{\Integerplus}{{{\Integer}^{+}}}
% \newcommand{\Realplus}{{{\Real}_{+}}}
% \newcommand{\meas}[1]{\mu\left(#1\right)}
% \newcommand{\as}{\ \text{a.e.}}
% \newcommand{\ess}{\mathrm{ess}}
% \newcommand{\sinc}{\mathrm{sinc}}
% \newcommand{\vphi}{\Ve{\phi}}
% \newcommand{\normx}[1]{\norm{#1}_{\Spc{X}}}
% \newcommand{\normy}[1]{\norm{#1}_{\Spc{Y}}}
% \newcommand{\ipx}[2]{\ip{#1}{#2}_{\Spc{X}}}
% \newcommand{\ipy}[2]{\ip{#1}{#2}_{\Spc{Y}}}
% \newcommand{\ltwo}{\ell_2(\Integer)}
% \newcommand{\lp}{\ell_p(\Integer)}
% \newcommand{\rep}[2]{[#1]_{#2}}
% \newcommand{\repop}[3]{\,\leftidx{_{#3}}{[{#1}]}{_{#2}}\,}
% %\newcommand{\valpha}{\boldsymbol{\alpha}}
% %\newcommand{\vbeta}{\boldsymbol{\beta}}
% %\renewcommand{\Conj}[1]{\overline{#1}}
% %\renewcommand{\Span}[1]{\text{Span}\left\{#1\right\}}
% \newcommand{\converge}{\rightarrow}
% \newcommand{\notconverge}{\not \rightarrow}
% \newcommand{\Close}[1]{\overline{#1}}
% \newcommand{\nin}{\not \in}
% \newcommand{\existsunique}{\exists!\ }
% \newcommand{\vd}{\Ve{d}}
% \newcommand{\Order}[1]{O(#1)}
% \newcommand{\BMF}{\mathrm{BMF}}
% \newcommand{\LMV}{\mathrm{LMV}}
% \newcommand{\Sig}[1]{\mathfrak{#1}}
% \newcommand{\Complement}[1]{{#1}^c}
% \newcommand{\Realpart}[1]{\Re(#1)}
% \newcommand{\Impart}[1]{\Im(#1)}
% \newcommand{\Nullset}{\emptyset}
% \newcommand{\Cov}[2]{\mathrm{Cov}(#1,#2)}
% \newcommand{\Var}[1]{\mathrm{Var}(#1)}
% \newcommand{\Cor}[2]{\mathrm{Cor}(#1,#2)}
% \newcommand{\vk}{\Ve{k}}
% \newcommand{\vdelta}{\boldsymbol{\delta}}
% \newcommand{\Card}[1]{\abs{#1}}
% \newcommand{\Gen}[1]{\mathrm{gen} (#1)}
% \newcommand{\HL}[1]{\color{orange} ( #1 ) \color{black}}

